A Lightweight Edge-CNN-Transformer Model for Detecting Coordinated Cyber and Digital Twin Attacks in Cooperative Smart Farming

The agriculture sector is increasingly adopting innovative technologies to meet the growing food demands of the global population. To optimize resource utilization and minimize crop losses, farmers are joining cooperatives to share their data and resources among member farms. However, while farmers benefit from this data sharing and interconnection, it exposes them to cybersecurity threats and privacy concerns. A cyberattack on one farm can have widespread consequences, affecting the targeted farm as well as all member farms within a cooperative. In this research, we address existing gaps by proposing a novel and secure architecture for Cooperative Smart Farming (CSF). First, we highlight the role of edge-based DTs in enhancing the efficiency and resilience of agricultural operations. To validate this, we develop a test environment for CSF, implementing various cyberattacks on both the DTs and their physical counterparts using different attack vectors. We collect two smart farming network datasets to identify potential threats. After identifying these threats, we focus on preventing the transmission of malicious data from compromised farms to the central cloud server. To achieve this, we propose a CNN-Transformer-based network anomaly detection model, specifically designed for deployment at the edge. As a proof of concept, we implement this model and evaluate its performance by varying the number of encoder layers. Additionally, we apply Post-Quantization to compress the model and demonstrate the impact of compression on its performance in edge environments. Finally, we compare the model's performance with traditional machine learning approaches to assess its overall effectiveness.

==> 7.Digitaltwinattack.tex <==
\section{Executing Attacks on Digital Twins at the Edge}

\label{sec:digitaltwin}
\begin{figure*}[!t]
\centering
\includegraphics[width=0.9\textwidth]{Digital twin application.png}
\caption{Use-case Demonstration of Coordinated Attack in DT in CSF.}
\label{fig:fig9}
\end{figure*}
This segment will exemplify the execution of attacks within a DT simulated at the edge. We first establish a DT at the edge to initiate the attack, as described in section~\ref{sec:testbed}. Then, a DT graph was generated using Azure Digital Explorer. Within this graph, we emulate various sensors utilized in \textit{Smart Farm A}. Subsequently, we execute an attack within DT, demonstrating its impact on the corresponding farms.

There are various possible attacks~\cite{karaarslan2021digital,alves2019digital} on DTs, where the attacker defeats the DTs' security by manipulating their behaviour or exploiting the update from the physical system to the DTs to steer the CSF into an insecure state. As shown in Figure.~\ref{fig:DT-attack}, We employ the model corruption technique to attack DT. The fundamental principle of a DT relies on maintaining synchronization between its physical and digital counterparts. If an attacker disrupts this synchronization, the DT model will deviate from its intended behaviour. For example, the attacker may sniff the network, gain access to the DT environment, inspect the code, and inject malicious code to corrupt the model. To accomplish this, we develop a malicious Python application that generates simulated data vastly different from the physical counterpart (Figure.~\ref{fig:DT-attack}). Consequently, the digital model becomes compromised, impacting the accuracy of the DT representation. As a result, the DT may no longer faithfully mirror its physical counterpart, leading to inconsistencies in output. The impact is easily visualized using the Grafana visualization tool. Figure \ref{fig:realIot} displays the real IoT sensor data, while Figure \ref{fig:simulated}
presents the DT data after the attack. Ideally, the IoT data and DT data should be identical; however, as shown, the DT data significantly deviates from the real IoT data.
\subsection{Impact of Attack on Digital twin in CSF}


Attacks on DTs can have far-reaching consequences for CSF. If a compromised DT interacts with shared data or resources within the smart farming network, it could introduce corrupted or manipulated data into the system.
To verify this, we present a brief use case (Figure \ref{fig:fig9}). In our use case scenario, each \textit{Smart Farm  A and B} has its DT model, which relies on data from real sensors. The DT model assists in predictive analysis and developing client applications for smart farming. \textit{Smart Farm A and B} share their DT data with the CSF per their contract.
Let's say another \textit{Smart Farm C} wants to build a smart irrigation model using the DT data from \textit{Smart Farm A and B}. The significance of DT data in the smart irrigation model is that it can predict future sensor data, allowing the system to implement IoT platforms and irrigation strategies before deployment in the field. It also enables the evaluation of different irrigation strategies that are parallel to current farm practices.

Using the strategies described above, an attacker manipulates \textit{Smart Farm A}'s DT data (Figure \ref{fig:DT-attack}). This manipulation introduces corrupted or false data into \textit{Smart Farm A}'s DT model. The compromised DT of Farm A continues to share its data to \textit{Smart Farm C}, which relies on the accuracy and integrity of \textit{Smart Farm A and B} data, and incorporates this corrupted data into its smart irrigation model.

The smart irrigation model in \textit{Smart Farm C} now works with corrupted data, leading to inaccurate predictions of soil moisture levels, weather conditions, and crop health. As a result, the model cannot accurately determine the optimal timing and volume for irrigation. This leads to inefficient water usage, either over- or under-irrigating crops, which can negatively impact crop yield and health (Figure \ref{fig:fig9}).

The corruption of the DT model in \textit{Smart Farm A} not only impacts itself but also severely undermines the efficiency of \textit{Smart Farm C}'s models and potentially other farms in the network that rely on shared data, directly impacting their operations. This demonstrates the cascading effect of a coordinated attack on DTs within a CSF network.





==> 8.Discussion.tex <==
\section{Discussion \& Finding}
\label{sec:discussion}

In the preceding section, we explore the impact of various network attacks within CSF. Additionally, we observe that attacks targeting the DT at the edge can disrupt its corresponding physical counterpart. This section will delve into several strategies to mitigate such cyberattacks.

\subsection{MITRE ATT\&CK Framework} 
MITRE ATT\&CK Framework is a documented knowledge base of malicious behaviour that threat attackers have used in real-world cyberattacks, referred to as techniques, tactics and behaviour \cite{mitre}. First released in 2013 and enhanced regularly over time, it aims to provide resources to the cybersecurity community to help them build resilience against attacks and develop confidence in their ability to mitigate vulnerability. The model is used globally by organizations across multiple cybersecurity disciplines, including threat modelling, intrusion detection, threat intelligence, and more.

In our proposed CSF testbed, we can use the MITRE ATT\&CK Framework in the edge(Windows) and cloud environments. This framework outlines various methods attackers might use to target cloud and edge systems. By understanding these tactics, farmers can enhance the security of their environments and better prevent data breaches and cyberattacks.
\subsection{Network Intrusion Detection System}

Another strategy for detecting cyber attacks is implementing a robust Network Intrusion Detection System (NIDS). This NIDS should be able to share attack and anomaly profiles with other smart farms, enhancing understanding and fostering versatile models capable of identifying various attack patterns and behaviours. Moreover, the NIDS model should possess the ability to adapt swiftly to new and evolving cyberthreats across all smart farms within the cooperative. For instance, if one smart farm encounters a novel cyberattack, the NIDS deployed in other smart farms should be capable of detecting this new attack. This analogy enables smart farms to detect zero-day attacks early, providing more time to respond and mitigate potential damage.
\subsection{zero-trust security}
The zero-trust security model operates on the principle of "never trust, always verify." This means that access to one area does not automatically grant access to all areas, and access granted at one time does not guarantee access at a different time.
To secure CSF, the zero-trust model requires users to provide valid credentials whenever they wish to access a system or resource. Verification is done through authentication (proving identity) and authorization (determining rights granted). Under the zero-trust model, these verifications are continuous, ensuring that users' credentials are validated at every access point and every time they request access. This approach ensures that even if users were trusted at a particular entry point or time, they must still revalidate their credentials for subsequent access.
\subsection{Web Application Firewall \& Network Firewall}

A Web Application Firewall (WAF) helps securing web applications by filtering and monitoring HTTP traffic between a web application and the internet. In our testbed, we simulated an attack targeting  traffic from physical sensors to the edge. By deploying a WAF at the network edge, we can filter traffic to the web application on the edge, thereby protecting against common vulnerabilities like SQL injection attacks.

On the other hand, a network firewall is software that restricts traffic flow between networks. Network firewalls help prevent cyberattacks by enforcing customized policies that block unauthorized traffic from accessing a secure network. In our testbed, we can secure the gateway router by enforcing customized policies at the edge.
While the AWS cloud includes default firewall services, additional security measures can be implemented by deploying these firewall services at the edge network, enhancing protection for our proposed test bed.

In CSF, integrating these advanced technologies at the edge of each smart farm can help detect and prevent cyberattacks. By implementing robust security measures and establishing a responsive isolation protocol, suspicious activity can be contained, preventing the spread of malicious data and safeguarding the entire network.
